DICE: Diversity in Deep Ensembles via Conditional Redundancy Adversarial Estimation

Deep ensembles perform better than a single network thanks to the diversity among their members. Recent approaches regularize predictions to increase diversity; however, they also drastically decrease individual members' performances. In this paper, we argue that learning strategies for deep ensembles need to tackle the trade-off between ensemble diversity and individual accuracies. Motivated by arguments from information theory and leveraging recent advances in neural estimation of conditional mutual information, we introduce a novel training criterion called DICE: it increases diversity by reducing spurious correlations among features. The main idea is that features extracted from pairs of members should only share information useful for target class prediction without being conditionally redundant. Therefore, besides the classification loss with information bottleneck, we adversarially prevent features from being conditionally predictable from each other. We manage to reduce simultaneous errors while protecting class information. We obtain state-of-the-art accuracy results on CIFAR-10/100: for example, an ensemble of 5 networks trained with DICE matches an ensemble of 7 networks trained independently. We further analyze the consequences on calibration, uncertainty estimation, out-of-distribution detection and online co-distillation.

==> tables/cifar10.tex <==
\begin{wraptable}{r}{}
\caption{\textbf{CIFAR-10 accuracy (Top-1)}.}%
\centering
\resizebox{0.4\textwidth}{!}{%
    \begin{tabular}{c|| c | c}
            \toprule
            \multirow{2}{*}{Name} & ResNet-32 & ResNet-110\\
             & 4-branch & 3-branch \\
            \midrule
            Ind. & 94.75\scalebox{.5}{$\pm$0.08} & 95.62\scalebox{.5}{$\pm$0.06} \\
            \midrule
            ONE & 94.41\scalebox{.5}{$\pm$0.05} & 95.25\scalebox{.5}{$\pm$0.08} \\
            OKDDip & 94.86\scalebox{.5}{$\pm$ 0.08} & 95.21\scalebox{.5}{$\pm$0.09} \\%
            \midrule
            ADP & 94.92\scalebox{.5}{$\pm$ 0.04} & 95.43\scalebox{.5}{$\pm$ 0.12} \\
            \midrule
            \midrule
            IB & 94.76\scalebox{.5}{$\pm$ 0.12} & 94.54\scalebox{.5}{$\pm$ 0.07} \\
            CEB &  94.93\scalebox{.5}{$\pm$ 0.11} & 94.65\scalebox{.5}{$\pm$ 0.05} \\
            \midrule
            IBR & 94.91\scalebox{.5}{$\pm$ 0.14} & 95.68\scalebox{.5}{$\pm$ 0.05} \\
            CEBR & 94.94\scalebox{.5}{$\pm$ 0.12} & 95.67\scalebox{.5}{$\pm$ 0.06} \\
            \midrule
            DICE & \textbf{95.01}\scalebox{.5}{$\pm$ 0.09} & \textbf{95.74}\scalebox{.5}{$\pm$ 0.08} \\
            \bottomrule
        \end{tabular}%
    }%
\label{table:cifar10}%
\end{wraptable}%

==> tables/cifar100robustness.tex <==
\begin{table}[ht]
\caption{\textbf{Uncertainty estimation} (NLL, BS) and \textbf{calibration} (ECE, TACE) on CIFAR-100.}
\centering
\resizebox{\textwidth}{!}{%
        \begin{tabular}{c  c || c | c c | c c || c c | c c | c }
            \cmidrule[0.4pt]{3-12}
            \multicolumn{2}{c|}{} & Temp. scaling & 1-net & Ind. & OKDDip-E & ADP & IB & CEB & IBR & CEBR & DICE \\
            \midrule
            Metrics & Unit & Temp. avg value & 1.49 & 1.31 & 1.33 & 0.64 & 1.21 & 1.24 & 1.17 & 1.19 & 1.11 \\
            \midrule
            Acc. $\uparrow$ & $\%$ & - & 71.28 & 76.71 & 76.85 & 77.21 & 76.93 & 76.98 & 77.25 & 77.30 & \textbf{77.51} \\
            NLL $\downarrow$ & $10^{-1}$ & \xmark/\cmark & 11.56/10.38 & 8.55/8.10 & 8.38/8.13 & 10.85/8.51  & 8.37/8.12 & 8.37/8.11 & 8.27/8.09 & 8.25/8.05 & \textbf{8.06}/\textbf{7.98} \\
            BS $\downarrow$ & $10^{-3}$ & \xmark/\cmark & 4.12/3.92 & 3.35/3.24 & 3.28/3.19 & 3.79/3.27 & 3.25/3.20 & 3.25/3.19  & 3.21/3.17 & 3.23/3.18 & \textbf{3.15}/\textbf{3.12}  \\
            ECE $\downarrow$ &  $10^{-2}$ & \xmark/\cmark & 10.47/1.83 & 7.45/\textbf{1.60} & 6.67/1.73 & 21.14/2.99 & 5.32/2.17 & 5.76/2.07 & 5.15/1.97 & 5.46/2.02 & \textbf{4.05}/2.59  \\
            TACE $\downarrow$ & $10^{-3}$ & \xmark/\cmark & 2.42/1.98 & 1.86/1.78 & 1.81/1.74 & 4.53/1.79 & 1.58/\textbf{1.68} & 1.67/1.69 & 1.60/1.75 & 1.65/1.72 & \textbf{1.46}/1.70  \\
            % \midrule
            % \multirow{5}{*}{CIFAR-100-C} & Acc. $\uparrow$  &\% & - & 43.67 & 48.23 & 47.19 & 49.01  & 48.39 & 48.45 & 48.71 & 48.74 & \textbf{49.34} \\
            % & NLL $\downarrow$  & $10^{-1}$ & \xmark/\cmark & 32.7/25.9 & 27.8/23.9 & 29.7/25.1 & \textbf{23.1}/24.6 & 26.8/24.3 & 27.3/24.8 & 26.21/24.38 & 25.78/24.76 & 25.6/\textbf{22.77} \\
            % & BS $\downarrow$ & $10^{-3}$ & \xmark/\cmark & 8.10/7.31 & 7.32/6.86 & 7.56/7.04 & \textbf{6.69}/6.91 & 7.19/6.88 & 7.26/6.88 & 7.09/6.83 & 7.08/6.95 & 6.93/\textbf{6.63} \\
            % & ECE $\downarrow$  & $10^{-2}$ & \xmark/\cmark & 27.9/13.8 & 23.2/14.0 & 24.83/15.29 & \textbf{7.59}/16.27 & 21.21/14.68 & 21.9/14.55 & 20.14/14.54 & 18.04/14.91 & 18.08/\textbf{13.47} \\
            % & TACE $\downarrow$ & $10^{-3}$ & \xmark/\cmark & 4.94/3.60 & 4.42/3.51 & 4.62/3.75 & 3.71/3.57 & 4.18/3.56 & 4.26/3.46 & 4.01/3.43 & 3.72/3.41 & \textbf{3.69}/\textbf{3.21}\\
            \bottomrule%
\end{tabular}%
}
\label{table:cifar100rob}
\end{table} 


==> tables/cifar10100full_backup.tex <==
\begin{table}[!ht]%
\caption{\textbf{Ensemble classification accuracy} (Top-1, \%) on \textit{CIFAR-100} and \textit{CIFAR-10}}%
\centering
\resizebox{1.0\textwidth}{!}{%
    \begin{tabular}{c| c c ||c c c c | c|c c | c c | c || c | c}
            \toprule
            \multicolumn{3}{c||}{Method} & \multicolumn{10}{c||}{CIFAR-100} & \multicolumn{2}{c}{CIFAR-10}\\
            \midrule
            \multicolumn{1}{c|}{Name} & \multicolumn{2}{c||}{Components} & \multicolumn{5}{c|}{ResNet-32} & \multicolumn{2}{c|}{Resnet-110} & \multicolumn{3}{c||}{WRN-28-2} & ResNet-32 & ResNet-110\\
             & Diversity & I.B. & 3-branches & 4-branches & 5-branches & 6-branches & 4-nets & 3-branches & 4-branches & 3-branches & 4-branches & 3-nets & 4-branches & 3-branches \\
            \midrule
            Ind. & & & 76.28 {\tiny $\pm$ 0.12} & 76.71 {\tiny $\pm$  0.19} & 77.17 {\tiny $\pm$  0.25} & 77.44 {\tiny $\pm$  0.16} & 77.38 {\tiny $\pm$  0.12} & 80.54 {\tiny $\pm$  0.09} & 80.76 {\tiny $\pm$  0.31} & 78.83 {\tiny $\pm$  0.12} & 79.10 {\tiny $\pm$  0.08} & 80.01 {\tiny $\pm$  0.15}  & 94.75 {\tiny $\pm$ 0.08} & 95.62 {\tiny $\pm$ 0.06} \\
            \midrule
            ONE-E \citep{NIPS2018_7980}& & & 75.17 {\tiny $\pm$ 0.35} & 75.13 {\tiny $\pm$ 0.25} & 75.25 {\tiny $\pm$ 0.22} & 75.32 {\tiny $\pm$ 0.28} & 76.25 {\tiny $\pm$ 0.32} & 78.97 {\tiny $\pm$ 0.24} & 79.86 {\tiny $\pm$ 0.25} & 78.38 {\tiny $\pm$ 0.45} & 78.47 {\tiny $\pm$ 0.32} & 77.53 {\tiny $\pm$ 0.36} & 94.41 {\tiny $\pm$ 0.05} & 95.25 {\tiny $\pm$ 0.08} \\
            OKDDip-E \citep{chen2020online}& Asym. Cod. & & 75.37 {\tiny $\pm$ 0.32} & 76.85 {\tiny $\pm$ 0.25} & 76.95 {\tiny $\pm$ 0.18} & 77.02 {\tiny $\pm$ 0.20} & 77.27 {\tiny $\pm$ 0.31}  & 79.07 {\tiny $\pm$ 0.27} & 80.46 {\tiny $\pm$ 0.35} & 79.01 {\tiny $\pm$ 0.19} & 79.32 {\tiny $\pm$ 0.17} & 80.02 {\tiny $\pm$ 0.14} & 94.86 {\tiny $\pm$  0.08} & 95.21 {\tiny $\pm$ 0.09} \\%
            \midrule
            ADP \citep{pang2019improving}& Non max. logits & & 76.37 {\tiny $\pm$ 0.11} & 77.21 {\tiny $\pm$ 0.21} & 77.67 {\tiny $\pm$ 0.25} & 78.17 {\tiny $\pm$ 0.14} & 77.51 {\tiny $\pm$ 0.25}  & 80.73 {\tiny $\pm$ 0.38} & 81.40 {\tiny $\pm$  0.27} & 79.21 {\tiny $\pm$ 0.19} & 79.71 {\tiny $\pm$ 0.18} & 80.01 {\tiny $\pm$ 0.17} & 94.92 {\tiny $\pm$  0.04} & 95.43 {\tiny $\pm$  0.12} \\
            \midrule
            \midrule
            IB & & VIB & 76.01 {\tiny $\pm$ 0.12} & 76.93 {\tiny $\pm$  0.24} & 77.22 {\tiny $\pm$ 0.19} & 77.46 {\tiny $\pm$ 0.16}  & 77.72 {\tiny $\pm$ 0.12} & 80.43 {\tiny $\pm$ 0.34} & 81.12 {\tiny $\pm$ 0.19} & 79.19 {\tiny $\pm$ 0.35} & 79.15 {\tiny $\pm$ 0.12} & 80.15 {\tiny $\pm$ 0.13} & 94.76 {\tiny $\pm$  0.12} & 94.54 {\tiny $\pm$  0.07} \\
            CEB & & VCEB & 76.36 {\tiny $\pm$ 0.06} & 76.98{\tiny $\pm$  0.18} & 77.35 {\tiny $\pm$ 0.14} & 77.68 {\tiny $\pm$ 0.04} & 77.64 {\tiny $\pm$  0.15}  & 81.08 {\tiny $\pm$  0.12} & 81.17 {\tiny $\pm$  0.16} & 78.92 {\tiny $\pm$ 0.08} & 79.20 {\tiny $\pm$ 0.13} & 80.38 {\tiny $\pm$ 0.18} & 94.93 {\tiny $\pm$  0.11} & 94.65 {\tiny $\pm$  0.05} \\
            \midrule
            IBMI (Ours \eqref{eq:libmi}) & MI & VIB & 76.68 {\tiny $\pm$ 0.13} & 77.25 {\tiny $\pm$  0.13} & 77.77 {\tiny $\pm$ 0.21} & 77.95 {\tiny $\pm$  0.13} & 77.84 {\tiny $\pm$ 0.12} & 81.34 {\tiny $\pm$ 0.21} & 81.38 {\tiny $\pm$  0.08} & 79.33 {\tiny $\pm$ 0.15} & 79.90 {\tiny $\pm$ 0.10} & 80.22 {\tiny $\pm$ 0.10} & 94.91 {\tiny $\pm$  0.14} & 95.68 {\tiny $\pm$  0.05} \\
            CEBMI (Ours \eqref{eq:lcebmi}) & MI & VCEB & 76.72 {\tiny $\pm$ 0.08} & 77.30 {\tiny $\pm$  0.12} & 77.81 {\tiny $\pm$  0.10} & 77.98 {\tiny $\pm$  0.15} & 77.82 {\tiny $\pm$  0.11}  & 81.52 {\tiny $\pm$ 0.11} & 81.55 {\tiny $\pm$ 0.33} & 79.25 {\tiny $\pm$ 0.15} & 79.98 {\tiny $\pm$ 0.07} & 80.35 {\tiny $\pm$ 0.15} & 94.94 {\tiny $\pm$  0.12} & 95.67 {\tiny $\pm$  0.06} \\
            \midrule
            DICE (Ours \eqref{eq:ldice})& CMI & VCEB & \textbf{76.89} {\tiny $\pm$  0.09} & \textbf{77.51} {\tiny $\pm$  0.17} & \textbf{78.08} {\tiny $\pm$  0.18} & \textbf{78.21} {\tiny $\pm$ 0.21} & \textbf{77.92} {\tiny $\pm$  0.08} & \textbf{81.67} {\tiny $\pm$ 0.14} & \textbf{81.93} {\tiny $\pm$  0.13} & \textbf{79.59} {\tiny $\pm$ 0.13} & \textbf{80.05} {\tiny $\pm$ 0.11} & \textbf{80.55} {\tiny $\pm$  0.12} & \textbf{95.01} {\tiny $\pm$  0.09} & \textbf{95.74} {\tiny $\pm$  0.08} \\
            \bottomrule
        \end{tabular}
    }%
\label{table:cifar10100full}%
\end{table}%

==> tables/determ_vs_ceb_small.tex <==
\begin{table}[!h]
\caption{\textbf{Comparison between deterministic and distribution encoders} on 4-branches ResNet-32.}
\centering
\resizebox{0.5\textwidth}{!}{%
        \begin{tabular}{c|c }
            \toprule
            Method & Top-1 (\%) accuracy on CIFAR-100\\
            \midrule
            Ind. & 76.78\scalebox{.8}{$\pm$ 0.19}\\
            Determ + CR no sampling & 77.09 \scalebox{.8}{$\pm$ 0.24}\\
            Determ + CR with sampling & 77.33 \scalebox{.8}{$\pm$ 0.21}\\
            DICE (VCEB + CR) & \textbf{77.51}\scalebox{.8}{$\pm$ 0.17} \\
            \bottomrule
        \end{tabular}
    }
\end{table}
